Robust Implementation of Retrieval-Augmented Generation on Edge-based Computing-in-Memory Architectures

Large Language Models (LLMs) deployed on edge devices learn through fine-tuning and updating a certain portion of their parameters. Although such learning methods can be optimized to reduce resource utilization, the overall required resources remain a heavy burden on edge devices. Instead, Retrieval-Augmented Generation (RAG), a resource-efficient LLM learning method, can improve the quality of the LLM-generated content without updating model parameters. However, the RAG-based LLM may involve repetitive searches on the profile data in every user-LLM interaction. This search can lead to significant latency along with the accumulation of user data. Conventional efforts to decrease latency result in restricting the size of saved user data, thus reducing the scalability of RAG as user data continuously grows. It remains an open question: how to free RAG from the constraints of latency and scalability on edge devices? In this paper, we propose a novel framework to accelerate RAG via Computing-in-Memory (CiM) architectures. It accelerates matrix multiplications by performing in-situ computation inside the memory while avoiding the expensive data transfer between the computing unit and memory. Our framework, Robust CiM-backed RAG (RoCR), utilizing a novel contrastive learning-based training method and noise-aware training, can enable RAG to efficiently search profile data with CiM. To the best of our knowledge, this is the first work utilizing CiM to accelerate RAG.

==> 1_intro-v0.tex <==
\section{Introduction}

The emerging Large Language Models (LLMs) are primarily deployed on centralized cloud computing platforms due to the overwhelming resource required. These cloud-hosted LLMs not only compromise user data privacy but also limited users' control over the model. This situation echoes the early days of computing when computers were room-sized machines accessible only in centralized locations. However, just as computers evolved to become personal and private tools, there is a clear pathway for LLMs to undergo a similar transformation. These intelligent AI systems, capable of generating customized responses to various user prompts, are poised to become personal, private intelligent tools. This evolution is not only a technological trend but is also driven by practical applications in fields such as medical, healthcare, companionship, and personal assisting, where data privacy and model reliability are paramount. The Edge LLM is becoming inevitable to satisfy these demoands.

To better fit distinct users needs, Edge LLMs need to learn from the interactions with users. However, the Edge LLMs learning is constrained by the limited resources of RAM and computational power. One common approach to enable Edge LLMs learning is to efficiently update parameters in \textit{q\_proj}, \textit{k\_proj}, \textit{v\_proj} (qkv) layers \cite{hu2021lora, dettmers2024qlora}. Such Parameter-Efficient Fine-Tuning (PEFT) methods can consume more than 60\% RAM and most the computational power for hours to update the model weights. Furthermore, PEFT requires professional labors to setup multiple hyper-parameters and prepossess the raw data into high-quality data to conduct an effective Edge LLM learning. 

\begin{figure}[h]
  \centering
  \includegraphics[width=0.9\columnwidth]{figures/fig_1.png}
  \caption{Learning curves of fine-tuning three different size Llama models on dataset LaMP-4, compared with the performance of two medium size Llama models under RAG, on the constraint of 8G RAM.}
  \label{fig:1}
\end{figure}

Different from PEFT, RAG can concatenate the user input text with the \textit{top\_k} relevant past user data to formalize a more informative prompt, which can lead the Edge LLMs to generate user-preferred content. Compared to PEFT, RAG neither consume limited resources to update the model weights nor take out the most computational powers for hours. As shown in Figure ~\ref{fig:1}, the preliminary study investigate Edge LLMs learning effectiveness of four different size variants of Llama \cite{touvron2023llama}. Given 8G RAM constraint, which commonly appears on edge devices such as Raspberry Pi and Jetson Orin, Llama2-3B-GPTQ with 2G model weights, TinyLlama-1.1B with 4G model weights, and Llama2-7B-GPTQ with 4G model weights can utilize PEFT to learn from dataset LaMP-4 \cite{salemi2023lamp}. Within 8 hours, Llama2-7B-GPTQ can achieve the best PEFT performance of 0.126 ROUGE-1 score. Differently, RAG allows a larger model Llama2-13B-GPTQ with 7G model weights to achieve 0.148 ROUGE-1 score without hours of model fine-tuning. Similarly, Llama-2-7B-GPTQ also can achieve 0.141 ROUGE-1 score under RAG, which is higher than its performance under PEFT.

Unfortunately, there exists three issues impeding RAG from being deployed on real-time user interaction with Edge LLMs. First, RAG commonly keeps the data and their embedded vectors (data embeddings) on RAM to enable fast response to the user input. The data embeddings is created by a sentence embedding model, where each piece of data consisting of several sentences are converted into vectors. In this paper, the data embeddings can be equivalent to sentence embeddings. Normally, the data and their embeddings are kept on RAM due to the data transfer cost when keeping them on disk. However, the RAM can limits the growing of user data, and its high \textbf{utilization} can lower resource allocated to the model. Furthermore, RAG performs Max Inner Product Search (MIPS) on the saved data embedding to rank their corresponding texts based on the semantic similarity, where the data most relevant to the current user input can be ranked top. On Raspberry Pi 4, one MIPS operation on a data space with 1500 data points can take up to 0.1s. Along with the usage of Edge LLMs, the user can accumulate millions of data points, where RAG can potentially cause non-negligible \textbf{latency} to minutes. Third, since the latency caused by MIPS constantly increases along with the accumulation of user data, it compromises the RAG \textbf{scalability} on large-scaled data space. 

Compute-in-Memory (CiM) has demonstrated its promising capabilities to alleviate high data movement costs while can perform massive parallel matrix multiplication operations in memory (\textcolor{red}{might want to specify what memory, how different from RAM}). By embedding CiM into RAG, the data embeddings can be saved on \textcolor{red}{(CiM memory)} and MIPS can find the relevant data embeddings on CiM without largely consume RAM and computational power. The CiM parallel computing can reduce the RAG latency. Additionally, compare to enlarge RAM, CiM can easily extend its memory space to save the growing user data. Finally, CiM can release RAG from competing the core computational resource.

However, simply embedding CiM into RAG cannot guarantee the benefit of CiM would not be compromised by its existing issues. Unlike the noise-tolerant RAM, where errors seldom occurs during writing the data embeddings, the error rate of writing data embeddings into CiM is negligible. If such errors are not mitigated, the corrupted data embeddings will accumulate on CiM. When perform MIPS on CiM, such corrupted data embeddings can cause MIPS find the data that are less relevant to the user input. Furthermore, the corrupted embeddings can mutually worsen the MIPS result during the parallel computing in CiM. 

To address this challenge, we propose a robust CiM-backed RAG framework to enable efficient RAG on large-scale user data. The framework consists of two stages: The first stage involves self-supervised training of the sentence embedding model to enhance its noise-resilience. We introduce noise-resilient sentence embedding model backed by contrastive learning to sharpen the distinctions within data embeddings while simultaneously decreasing their sensitivity to noise. \textcolor{red}{[need verify]: Additionally, due to the inherent structure and design of CiM, we incorporate compression and quantization within the noise-aware contrastive learning process. This adaptation shapes the data embeddings to meet specific requirements for efficient computation in CiM environments.} Collectively, this approach yields noise-resilient data embeddings optimized for efficient CiM computation.
% To address this challenge, we propose an robust CiM-backed RAG framework to enable efficient RAG on large-scale user data. This framework has two stages. The first stage is self-supervised training on the data embedding model to enhance the noise-resilient capability of data embedding. Noise-awared contrastive learning is proposed to increase the distinctions among the data embedding while reduce the noise sensitivity of the data embedding. \textcolor{red}{[need verify]}Also, due to the internal structure and design of CiM, compression and quantization are added to the noise-awared constrastive learning process to shape the data embedding to satisfy certain CiM efficient compution. Together, the noise-awared contrastive learning can produce noise-resilient data embedding that can satisfy CiM efficient computation.

The second stage is write-verify the certain data embeddings. While the noise-resilient sentence embedding model enhances the embedding robustness, this model cannot impact the errors occurring during CiM writing. To mitigate the error impact, we apply the write-verify on the semantic similar data embeddings which are nearby to each other decided by K-means. 

In summary, the main contributions of this work include:
\begin{itemize}
    \item \textbf{CiM-backed RAG framework towards Edge LLMs.} We are the first work to harvest the CiM advantage to accelerate the Edge LLMs. We provide a pathway to utilize emerging devices to expand the Edge LLMs capability. Our proposed framework can reduce the Edge LLMs latency, allow the wider scalability on the large-scaled user data, and release the resource burden from trivial data saving tasks.
    \item \textbf{Tailor the data embeddings to adapt CiM.} We propose a self-supervised training method to shape the data embeddings in two aspects: 1. Enhance the internal noise-resilient capability of the data embeddings, 2. Adjust the dimension and precision of the data embeddings via compression and quantization to enable CiM efficient computation of the data embeddings.
    \item \textbf{Reduce the data embeddings writing error.} We utilize write-verify on certain data embeddings to enhance the robustness of noise-sensitive embeddings.
\end{itemize}


==> 1_intro-v1.tex <==
\section{Introduction}

% LLM on edge device is important, 
% One way to do it is by RAG

% CiM on MIPS is doable and efficient

Retrieval-augmented generation (RAG) has become the de facto technique for enhancing the accuracy and reliability of language models \textcolor{red}{[cite]} through fact-based augmentation of user queries. In the era of Large Language Models (LLMs), compared to previous state-of-the-art (SOTA) models such as BERT \textcolor{red}{[cite]}, RoBERTa \textcolor{red}{[cite]}, and GPT2 \textcolor{red}{[cite]}, LLMs have demonstrated substantial improvements in reasoning capabilities, with increases from \textcolor{red}{xx} to \textcolor{red}{xx} \textcolor{red}{[cite]}. Given a user query, RAG enables LLMs refer the most relevant past user data to generate the user-preferred responses based on both past data and the current query.


While LLMs are predominantly deployed on cloud servers, there is a growing need to deploy them on edge devices (Edge LLMs), specifically for exclusive use by device owners. This deployment ensures complete user data privacy and control over the LLMs. Edge LLMs have potential applications in various fields, including medical \textcolor{red}{[cite]}, healthcare \textcolor{red}{[cite]}, companionship \textcolor{red}{[cite]}, and personal assistance \textcolor{red}{[cite]}. However, these models need to continuously learn from user data to adapt to previously unseen situations. Nevertheless, Edge LLMs face significant challenges due to limited resources, which constrains their ability to learn from user data.

\textcolor{red}{[there are many works accelerate edge LLM. but no work acclerate RAG]}

We foresee that the implementation of RAG will become increasingly prevalent, enabling Edge LLMs to learn from users effectively. By using RAG, Edge LLMs only need to store past user data and retrieve the most relevant data in response to user queries. Additionally, the current user query, along with the contextual conversation, can be archived and subsequently utilized as material for future interactions. Furthermore, Edge LLMs do not require overwhelmingly large resources from the edge device to update their parameters, ensuring that the utilization of RAG does not compromise the performance of other applications on the device. Considering both effectiveness and resource efficiency, RAG is well-suited to enable Edge LLMs to learn from users.

Unfortunately, there is currently not much work on the implementation of RAG onto resource-constrained edge devices. There exists three issues impeding RAG from being deployed on real-time user interaction with Edge LLMs. First, RAG commonly keeps the data and their embedded vectors (data embeddings) on RAM to enable fast response to the user input. The data embeddings is created by a sentence embedding model, where each piece of data consisting of several sentences are converted into vectors. In this paper, the data embeddings can be equivalent to sentence embeddings. Normally, the data and their embeddings are kept on RAM due to the data transfer cost when keeping them on disk. However, the RAM can limits the growing of user data, and its high \textbf{utilization} can lower resource allocated to the model. Furthermore, RAG performs Max Inner Product Search (MIPS) on the saved data embedding to rank their corresponding texts based on the semantic similarity, where the data most relevant to the current user input can be ranked top. On Raspberry Pi 4, one MIPS operation on a data space with 1500 data points can take up to 0.1s. Along with the usage of Edge LLMs, the user can accumulate millions of data points, where RAG can potentially cause non-negligible \textbf{latency} to minutes. Third, since the latency caused by MIPS constantly increases along with the accumulation of user data, it compromises the RAG \textbf{scalability} on large-scaled data space. 

Computing-in-Memory (CiM) architectures have shown substantial promise in accelerating matrix-vector multiplication, a common operator for many deep neural networks. The CiM architectures often utilize massive parallel processing to perform computations directly within the memory array where the data is stored, such that they can minimize the data movement through in-situ data access and significantly increase the throughput \cite{sze2017efficient}. Furthermore, by incorporating non-volatile memory (NVM) devices, such as phase-change memories (PCMs), resistive random-access memories (RRAMs), and ferroelectric field-effect transistors (FeFETs), CiM can outperform conventional MOSFET-based designs in terms of energy efficiency \cite{chen2016eyeriss}. However, it remains unknow whether the CiM architectures can be utilized to benefit RAG on Edge LLMs.


We notice that the core operation in RAG, which differs from that in deep neural networks, is not the matrix-vector operation but the Max Inner Product Search (MIPS) \textcolor{red}{[cite]}. Initially, a user query is textual data that is embedded into a vector by a sentence embedding model. Similarly, each document in the past user data is stored as vectors. The vectors can also be called as embeddings. MIPS calculates the inner product between the vector of the user query and those of each document. The higher the product, the greater the semantic similarity between the user query and the corresponding document. MIPS ranks these products from highest to lowest and returns the document with the top products. 

Therefore, we propose to leverage CiM architecture in a new way so that it can be used to accelerate MIPS, the document embeddings are saved into the matrix representation of CiM, and the user query embedding is used as the vector representation of CiM. In CiM, each memory cell can store an element of a embedding, allowing the simultaneous computation of multiple products across the vector elements. By activating the appropriate rows and columns in the memory array, CiM can calculate the dot product of two embeddings by summing the products of corresponding elements, all within the memory itself. The latency of MIPS will be proportional to data size but only related to the performance of parallel processing capability of CiM. In this way, CiM can significantly reduce the MIPS latency. \textcolor{red}{[a very short sentence would be enough]}

\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figures/fig_3.png}
  \caption{MIPS performance of RAG given different noise level on the data embedding.}
  \label{fig:prelim}
\end{figure}

Unfortunately, such a direct application of CiM for RAG is not enough, and it will greatly deteriorate the RAG performance for several reasons:
\begin{itemize}
    \item CiM is not efficient to support high-resolution multiplication, and it is good for low resolution computing. CiM architectures are inherently limited by the precision of the analog computation, affected by the variability of NVMs and noise. However, as the accumulation of user data, many embeddings can be semantic similar. The low resolution may not precisely represent these embeddings and lead MIPS to have wrong results.
    % why CiM is not good to high resolution, how much bits

    \item Repeated modifying CiM’s content (i.e., writing new weight values) will gradually change the values. Frequent updates to the weights stored in CiM can lead to degradation of the memory cells. Each write operation can slightly alter the electrical characteristics of the cells, leading to drift in the stored values over time. This could also compromise the MIPS results.
    % some termnologies are wrong, drift. 
    \textcolor{red}{[could drop]}
    
    \item The operations performed in CiM architectures are susceptible to various sources of noise, including electronic noise (thermal, shot, and flicker), device-to-device variability, and line noise from the supporting circuitry. These noise sources can corrupt the computations, especially when the signal levels are close to the noise floor, which is a common scenario in high-precision tasks. Such noise issues are critical in RAG applications where the accuracy and quality of the generated content heavily rely on the precision of the underlying computations.

    \item These CiM-specific characteristics significantly impact MIPS performance. As shown in Figure~\ref{fig:prelim}, a preliminary study on the effect of noise on MIPS across five datasets has demonstrated that noise can substantially affect MIPS performance. As the noise level increases, MIPS accuracy can drop dramatically, approaching \(0\). \textcolor{red}{[need to detail to the setting]}

\end{itemize}


Therefore, we propose a novel optimization framework for RAG so that it can be robustly implemented onto CiM. The framework consists of three parts. The first part is an end-to-end optimization of RAG to address the noise issues of CiM. For various CiM architectures, their NVM devices may exhibit different ranges of noise and be compatible with specific array sizes, which necessitates that embeddings be shaped to certain lengths and precisions. Our framework optimizes RAG performance and enables it to adapt to all types of CiM architectures. The second part is a contrastive learning approach to train the embedding model for RAG. User data may either be explicitly labeled by users to indicate preferences or left as pure informational statements without labels specifying user preferences. Contrastive learning is an effective method to enhance the performance of the embedding model, whether using labeled or unlabeled data \textcolor{red}{[cite]}. In contrastive learning, we modify the triplet loss training objective to fit with our designed data augmentation methods. The third part is new data augmentation methods to deal with labeled and unlabled data respectively. Our methods can automatically create triplets that highlight the distinction of every single embedding. The contrastive learning trained by these constructed data can improve the robustness of RAG's implementation on CiM.


The major contributions of our work can be summarized as:

\textcolor{red}{[we accelerate rag instead of Edge LLM]}
\begin{itemize}
    \item \textcolor{red}{We are the first work to harvest the CiM advantage to accelerate the Edge LLMs. We provide a pathway to utilize emerging devices to expand the Edge LLMs capability. Our proposed framework can reduce the Edge LLMs latency, allow the wider scalability on the large-scaled user data, and release the resource burden from trivial data saving tasks.}
    \item We introduce an optimization method to adapt RAG onto many CiM architectures. With knowing the noise features and hardware requirements of the CiM architectures, our method can efficiently learn to reshape the embeddings to minimize the CiM constraints impact.
    \item Our experiments on multiple datasets show that the proposed framework achieves up to \textcolor{red}{xx}\% higher performances than baselines under the same CiM architectures.
    \item \textcolor{red}{[can add a few more points based on results]}
\end{itemize}

The structure of this paper unfolds as follows: In section 2, we xxx. In Section 3, we xxx. In section 4, we xxx. In section 5, we xxx. 


==> 1_intro_v2.tex <==
\section{Introduction}

% LLM on edge device is important, 
% One way to do it is by RAG

% CiM on MIPS is doable and efficient

The emerging Large Language Models (LLMs) deployed primarily on centralized cloud platforms (Cloud LLMs), raising concerns about user privacy and trustworthy issues \cite{neel2023privacy}. The Cloud LLMs mirror the early days of computers when such large machines dominated centralized locations. But, just as personal computers evolved, LLMs are poised to follow suit. The Cloud LLMs, capable of generating customized responses, will eventually transition into personalized LLMs deployed on edge devices (Edge LLM). This evolution is not only a technological trend but also driven by practical needs in areas such as healthcare, companionship, and personal assistance, where privacy and reliability are crucial \textcolor{red}{[cite]}. The emergence of Edge LLMs is inevitable to meet these demands.


To better suit the needs of individual users, Edge LLMs must learn from user interactions. However, their learning is constrained by limited RAM and computational power. Similar to Cloud LLMs, the Edge LLMs primarily learn by updating their model parameters. Yet, given that these models often contain over 3 billion parameters, updates can be challenging. While the efforts to accelerate Edge LLMs learning \cite{qin2023enabling} \textcolor{red}{[more cites]} have been made, such works still requires overwhelming huge resource from the edge devices while preventing other programs to properly function. For example, the pockengine \cite{zhu2023pockengine} can take around 9 hours to train the model on a dataset of 5,000 documents using a high-performance embedded system like the Nvidia Jetson AGX Orin, making this option impractical for regular users due to its cloud-resource-equivalent cost. Retrieval-augmented generation (RAG) offers an alternative, emerging as the de facto learning method for Edge LLMs due to its lower resource demands \textcolor{red}{[cite]}. RAG retrieves documents relevant to the user's query from past user data, providing more informative input without needing to update model parameters.


We foresee that the implementation of RAG will become increasingly prevalent, enabling Edge LLMs to learn from users effectively. However, there exists three issues impeding RAG from being deployed on real-time user interaction with Edge LLMs. First, RAG commonly keeps the past user data on RAM to enable fast response to the user input. However, the RAM can limits the growing of user data, and its high utilization can lower resource allocated to the model. Furthermore, RAG performs Max Inner Product Search (MIPS) on the saved data embedding to rank their corresponding texts based on the semantic similarity, where the data most relevant to the current user input can be ranked top. On Raspberry Pi 4, one MIPS operation on a data space with 1500 data points can take up to 0.1s. Along with the usage of Edge LLMs, the user can accumulate millions of data points, where RAG can potentially cause non-negligible latency to minutes. Third, since the latency caused by MIPS constantly increases along with the accumulation of user data, it compromises the RAG scalability on large-scaled data space. 

Unfortunately, there are few efforts have been made to optimize RAG towards the Edge LLMs. We notice that the core operation in RAG, MIPS, is actually an vector multiplication. For MIPS, it stores every document from the past user data into a numerical array, created by an sentence embedding model. MIPS operates the vector multiplication between each document and the current user query. The document with largest product will be selected. We find that such vector multiplications can happen to be accelerated by Computing-in-Memory (CiM) architectures.

\begin{figure}[h]
  \centering
  \includegraphics[width=0.8\columnwidth]{figures/fig_3.png}
  \caption{MIPS performance of RAG given different noise level on the data embedding.}
  \label{fig:prelim}
\end{figure}

CiM architectures have shown substantial promise in accelerating matrix-vector multiplication, a common operator for many deep neural networks. The CiM architectures often utilize massive parallel processing to perform computations directly within the memory array where the data is stored, such that they can minimize the data movement through in-situ data access and significantly increase the throughput \cite{sze2017efficient}. Furthermore, by incorporating non-volatile memory (NVM) devices, such as phase-change memories (PCMs), resistive random-access memories (RRAMs), and ferroelectric field-effect transistors (FeFETs), CiM can outperform conventional MOSFET-based designs in terms of energy efficiency \cite{chen2016eyeriss}. 

Therefore, we propose to leverage CiM architecture to optimize RAG. Given the parallel processing capabilities of the CiM architecture, and that its operation will not compete for core computational resources with other edge programs \cite{yang2020co}, the CiM architecture can reduce RAG latency and enhance RAG scalability over large-scale data spaces. Unfortunately, such a direct application of CiM for RAG is not enough, and it will greatly deteriorate the RAG performance for several reasons.

First, The CiM was primarily designed and optimized for low-resolution computing \textcolor{red}{[cite]}. However, in RAG, it requires that user data documents have embeddings as FP32 precision with over 128 dimensions, which can precisely represent the semantic meanings of these documents \textcolor{red}{[cite]}. The low resolution of CiM, with typically 64 x 64 arrays, may not precisely represent these embeddings and may lead MIPS to produce incorrect results.

Then, The operations performed in CiM architectures are susceptible to various sources of noise, including electronic noise (thermal, shot, and flicker), device-to-device variability, and line noise from the supporting circuitry. These noise sources can corrupt the computations, especially when the signal levels are close to the noise floor, which is a common scenario in high-precision tasks. Such noise issues are critical in RAG applications where the accuracy and quality of the generated content heavily rely on the precision of the underlying computations.

Additionally, we present a preliminary study to demonstrate the impact of CiM-specific characteristics on MIPS performance as shown in Figure ~\ref{fig:prelim}. We use a CiM device RRAM, whose device variation can be found in Table ~\ref{tab:var}, and examine different level of device variations, \emph{i.e.}, different $\sigma$ values in the Gaussian noise model shown in equation ~\ref{eq:dev_var}. We evaluate MIPS performance by comparing its retrieved results without device variation to those under device variation. As the noise level increases, MIPS accuracy can drop dramatically, approaching random guessing.

To enable CiM into optimize the RAG, therefore, we propose a novel optimization framework for CiM-backed RAG. The framework consists of three parts. The first part is an end-to-end optimization of RAG to address the noise issues of CiM. For various CiM architectures, their NVM devices may exhibit different ranges of noise and be compatible with specific array sizes, which necessitates that embeddings be shaped to certain lengths and precisions. Our framework optimizes RAG performance and enables it to adapt to all types of CiM architectures. The second part is a contrastive learning approach to train the embedding model for RAG. User data may either be explicitly labeled by users to indicate preferences or left as pure informational statements without labels specifying user preferences. Contrastive learning is an effective method to enhance the performance of the embedding model, whether using labeled or unlabeled data \textcolor{red}{[cite]}. In contrastive learning, we modify the triplet loss training objective to fit with our designed data augmentation methods. The third part is new data augmentation methods to deal with labeled and unlabled data respectively. Our methods can automatically create triplets that highlight the distinction of every single embedding. The contrastive learning trained by these constructed data can improve the robustness of RAG's implementation on CiM.


The major contributions of our work can be summarized as:

\textcolor{red}{[we accelerate rag instead of Edge LLM]}
\begin{itemize}
    \item We are the first work harvesting CiM advantages to accelerate RAG. In this way, We provide a pathway to utilize emerging devices to expand the Edge LLMs capability.
    \item Our proposed framework can reduce the Edge LLMs latency, allow the wider scalability on the large-scaled user data, and release the resource burden from trivial data saving tasks.
    \item We introduce an optimization method to adapt RAG onto many CiM architectures. With knowing the noise features and hardware requirements of the CiM architectures, our method can efficiently learn to reshape the embeddings to minimize the CiM constraints impact.
    \item Our experiments on multiple datasets show that the proposed framework achieves up to \textcolor{red}{xx}\% higher performances than baselines under the same CiM architectures.
    \item \textcolor{red}{[can add a few more points based on results]}
\end{itemize}

\textcolor{red}{The structure of this paper unfolds as follows: In section 2, we xxx. In Section 3, we xxx. In section 4, we xxx. In section 5, we xxx. }


==> 2_related_v0.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figures/fig_2.png}
  \caption{The workflow of CiM-backed RAG}
  \label{fig:2}
\end{figure}

\section{Related Work}
% \subsection{Contrastive Learning}

% % \subsubsection{\textbf{Contrastive Learning}}

% In natural language processing (NLP), contrastive learning like \textit{SimCSE} \cite{chen2020simple} aims to learn feature representations by pulling semantically similar representations closer and pushing semantically dissimilar representations apart. Given the dataset \(\mathcal{D} = \{x_i\}_{i=1}^s\) where \(i = 1, 2, ..., s\), this method employs a set of paired examples \( \mathcal{D}' = \{(x_i, x^+_i)\}_{i=1}^s \), where \( x_i \) and \( x^+_i \) are semantically related. Using a cross-entropy loss function with in-batch negatives, the approach fine-tunes pretrained models like BERT \cite{devlin2018bert} and RoBERTa \cite{liu2019roberta}. Specifically, let \( p_i \) and \( p^+_i \) denote the representations of \( x_i \) and \( x^+_i \) respectively. The training objective for a mini-batch of \( N \) pairs is given by 

% \begin{equation}
% \mathcal{L} = -\log \frac{e^{\text{sim}(p_i, p^+_i)/\tau}}{\sum_{j=1}^N e^{\text{sim}(p_i, p_j)/\tau}},     
% \end{equation}
% where \( \tau \) is a temperature hyperparameter and \(sim(p_1, p_2)\) is the cosine similarity \(\frac{p_1^\top p_2}{\|p_1\| \|p_2\|}\). 

% Different from the cross-entropy loss commonly used in contrastive learning, we follow the large margin nearest neighbor (LMNN) by Weinberget et al. \cite{weinberger2005distance}: let $x_i$ to be an anchor example, with its corresponding negative example $x^-$ and positive example $x^+$, where $x^i$ is closer to $x^+$ compared to $x^-$. They formalize a set of triple examples \(\mathcal{D}_{t} = \{(x_i, x^-_i, x^+_i)\}_{i=1}^s \). For the margin $m$, the triplet loss objective for a mini-batch of \(N\) triple examples is given by

% \begin{equation}
% \mathcal{L}' = \sum_{i=1}^N \max \left(0, \text{d}(p_i, p^-_i) - \text{d}(p_i, p^+_i) + m\right)
% \end{equation}
% where
% \begin{equation}
%     \text{d}(p_a, p_b) = ||p_a - p_b||
% \end{equation}
% calculates the norm degree for pairwise distance. 
% In this work, we will modify the triplet loss $\mathcal{L}'$ to align it with our constructed textual data.



% \textcolor{yellow}{In this work, different from the cross-entropy loss function used by SimCSE, we take a triplet loss function \cite{khosla2020supervised}: let $x_{i}$ to be the anchor examples, with their corresponding negative examples $x^-$ and positive examples $x^+$, formalize a set of triple examples \(\mathcal{D}^{t} = \{(x_i, x^-_i, x^+_i)\}_{i=1}^s \). Utilizing the \(sim(h_1, h_2)\), we calculate \(sim^+\) and \(sim^-\) and use margin \(m\) to confine the decrease of \(sim^+\) and the increase \(sim^-\). The training object for a mini-batch of \(N\) pairs is given by:
% \begin{equation}
% \mathcal{L}^t = \frac{1}{N} \sum_{i=1}^N \frac{1}{1 + e^{-\left(\text{sim}(h_{i}, h_{i}^-) - \text{sim}(h_{i}, h_{i}^+) + m\right)}},
% \label{eq:2}
% \end{equation}
% where \( h_{i} \), \( h_{i}^+ \), and \( h_{i}^- \) are the embeddings for the anchor, positive, and negative examples of the \(i\)-th pair in the batch, respectively. The equation ~\ref{eq:2} will be used to finetune the sentence embedding model parameters in this work.}

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\columnwidth]{figures/fig_2.png}
%   \caption{The workflow of CiM-backed RAG}
%   \label{fig:2}
% \end{figure}

% \begin{figure*}[h]
%   \centering
%   % First row of figures
%   \begin{subfigure}[b]{0.38\textwidth}
%     \includegraphics[width=1\textwidth]{figures/fig_3.png}
%     \caption{Noise $\sigma = [0.0, 0.6]$}
%     \label{fig:fig_3}
%   \end{subfigure}
%   % \hfill % space between the subfigures
%   \begin{subfigure}[b]{0.27\textwidth}
%     \includegraphics[width=1\textwidth]{figures/fig_3_b.png}
%     \caption{Compress $\sigma = (0.0, 0.1)$}
%     \label{fig:fig_3_b}
%   \end{subfigure}
%   % \hfill % space between the subfigures
%   \begin{subfigure}[b]{0.155\textwidth}
%     \includegraphics[width=1\textwidth]{figures/fig_3_c.png}
%     \caption{Quantize $\sigma = 0.0$}
%     \label{fig:fig_3_c}
%   \end{subfigure}
%   % Second row of figures
%   \begin{subfigure}[b]{0.157\textwidth}
%     \includegraphics[width=1\textwidth]{figures/fig_3_d.png}
%     \caption{Quantize $\sigma = 0.1$}
%     \label{fig:fig_3_d}
%   \end{subfigure}
%   \caption{Information retrieval performance of RAG given (a) different noise level on the data embedding. When we compress the data embedding, (b) noise can have intensive impact on compressed data embedding. When we quantize the data embedding, (c) without noise, the RAG preforms poorly, and (d) with noise, the RAG has even worse performance.}
%   \label{fig:prelim}
% \end{figure*}

% prelimrary
%         ds1 ds2 ds3 ds4 
% cim1
% cim2
% cim3
% cim4

% if train
% unsuper

% super
% baselins
% ours



% \subsubsection{\textbf{FeFET-based CiM}}
\subsection{CiM Architectures and their NVMs}

The core building block of nvCiM MIPS accelerators is the crossbar array architecture. As shown in the middle part of Figure~\ref{fig:2}, this array is the computational unit for matrix-vector multiplication. In this array, matrix values, which are \todo{data embeddings} if used in a CiM RAG accelerator, are stored at the cross-points of vertical and horizontal lines through emerging technologies like FeFETs. Simultaneously, vector values, which are \todo{query embeddings} in a CiM RAG accelerator, flow along the horizontal lines of the array. Operations within the crossbar take place in the analog domain. However, for other essential functions like shift-and-add for multiple bits and sorting to find the top-k fit should be done in the digital domain. Thus, digital-to-analog and analog-to-digital converters are used to connect these different components.

Crossbar arrays suffer from various sources of variations and noises. Two major ones include spatial variations and temporal variations. Spatial variations result from fabrication defects and have both local and global correlations. FeFET devices also suffer from temporal variations due to the stochasticity in the device material, which causes fluctuations in conductance when programmed at different times. Temporal variations are typically independent from device to device and are irrelevant to the value to be programmed~\cite{feinberg2018making}.   
In this work, as a proof of concept, we focus on the impact of temporal variations in the programming process on DNN performance. Temporal variation makes the programmed resistance of a device deviate from what is expected. The proposed framework can also be extended to other sources of variations with modification.

Experimental results~\cite{yan2022swim, yan2021uncertainty} show that the noise on DNN weights caused by device variations can be safely modeled as a Gaussian noise with zero mean, each with a standard deviation associated with the weight value. A detailed representation is:
\begin{equation}\label{eq:dev_var}
    \mathbf{v} = \mathbf{v_0} + \Delta\mathbf{v}, \Delta\mathbf{v}\sim\mathcal{N}(0,\sigma_v)
\end{equation}
where $\mathbf{w}$ is the actual embedding deployed on the accelerators, $\mathbf{v_0}$ is the target embedding value, and $\sigma_v$ is a value measured by the experiments. We collect the measurement results from RRAM and FeFET devices and the specific value will be discussed in section \todo{XXX}.



% \begin{itemize}
%     \item \textcolor{blue}{[Zheyu] One short paragraph to further explain relation between CiM architecture and NVM} In our work, the noise and error comes from NVM? And one cim arch can correspond to one NVM
%     \item \textcolor{blue}{[Zheyu] In intro, I include PCMs, RRAMs, and FeFETs. We might need to give each of them 1 to 3 sentences. Using the formula, explain the five noise pattern, and how they comes}
%     \begin{itemize}
%         \item CiM1: \{1,1,1,1\}
%         \item CiM2: \{1,2,2,1\}
%         \item CiM3: \{1,4,4,1\}
%         \item CiM4: \{1,6,6,1\}
%         \item CiM5: \{1,3,3,1\}    
%     \end{itemize}
% \end{itemize}

\begin{figure*}[t]
  \centering
  \includegraphics[width=0.9\textwidth]{figures/fig_5.png}
  \caption{Overview of the framework. Train the noise-resilient sentence transformer under our contrastive learning method. }
  \label{fig:framework}
\end{figure*}

\subsection{Past noise mitigation methods}
% \textcolor{blue}{[Zheyu], maybe you can give a short explain of the past mitigation method here. Later, we can decide whether they should be placed in section 2 to section 4 under "baseline"}

Several strategies have been introduced to tackle the challenge of device variations in CiM DNN accelerators. This section briefly discusses the two predominant approaches: bolstering DNN robustness and curtailing device variations.

A prevalent technique to bolster DNN robustness in the face of device variations is variation-aware training\cite{jiang2020device,peng2019dnn+,he2019noise,chang2019nv}. This method, sometimes referred to as noise-injection training, integrates variations into DNN weights during the training phase. This integration fosters a DNN model that exhibits statistical resilience to the effects of device variations. In each training iteration, a variation instance, drawn from a predefined distribution, augments the weights during the forward pass, leaving the backpropagation phase unaffected by noise. Upon gradient collection, this variation is discarded, and the pristine weight is updated based on the accrued gradients. Alternatives encompass the design of sturdier DNN architectures~\cite{jiang2020device, yan2021uncertainty, gao2021bayesian} and pruning techniques~\cite{jin2020improving, chen2021pruning}.

In efforts to decrease device variations, the write-verify procedure \cite{shim2020two, yao2020fully} is commonly employed during programming. Initially, an NVM device is programmed to a set state via a designated pulse pattern. Subsequent to this, the device's value is verified to ascertain if its conductance aligns with a stipulated range of the desired value, essentially assessing its accuracy. If discrepancies arise, a supplemental update pulse is initiated to draw the device conductance nearer to the target. This loop persists until the disparity between the programmed device value and the target diminishes to a satisfactory margin, typically taking a handful of cycles. Cutting-edge research suggests that by selectively applying write-verify to a subset of pivotal devices, one can uphold the average accuracy of a DNN \cite{yan2022swim}. Additionally, a variety of circuit design initiatives~\cite{shin2021fault, jeong2022variation} have been put forth to counteract device variations.






% \textcolor{blue}{[TO DO - Compression and Quantization]}

% original dim: 384
% compress: 256, 128, 64, 32, 16
% quantization: int8, uint8, binary, ubinary

% fefet device1: 128 + int8
% 1 6

% \textcolor{red}{we want to specify in what cases, we need compression and quantization, need some details.}

\subsection{Retrieval-Augmented Generation (RAG)}

% \subsubsection{\textbf{Retrieval-Augmented Generation (RAG)}}
Retrieval-augmented generation (RAG) is a cutting-edge technique revolutionizing the usage of LLMs. It is a well-known issue that LLMs will hallucinate during inference \cite{huang2023survey}, and RAG could reduce such hallucinations via providing grounded context that is presented in a knowledge base.
When an LLM system takes a user prompt as its input, RAG will assist the system to search for prompt-relevant content in its user database, concatenate the original user query with the searched content to form a more informative prompt, and generate response based on the new informative prompt \cite{lewis2020retrieval}. As shown in Figure ~\ref{fig:2}, every data in user database will be converted into sentence embeddings via a sentence embedding model, and an embedding space will be formed with these sentence embeddings that are saved \textcolor{red}{into certain locations, in our case, CiM}. 

Previously, researches on applications of edge LLMs primarily focused on the either the retrieval model or the LLM aspects of the system. Common variations of the retrieval model include retrieval index optimization \cite{sarthi2024raptor, wang2023knowledge}, automatic query optimization \cite{dhuliawala2023chainofverification, kulkarni2024reinforcement}, and embedding model optimization \cite{li2023angleoptimized}. Other works related to LLM's usage of the retrieved context include context grounding \cite{qian2024grounding,lozano2023clinfoai} and even fine-tuning \cite{lin2024radit}. We refer readers to works from Gao et. al. \cite{gao2024retrievalaugmented} for a full review related to RAG optimizations.  However, to the best of authors' knowledge, no attention was drawn on the practical problems that will emerge during edge computing, which we argue to be pivotal for the success of edge RAG system.

%RAG typically utilizes an information retrieval method, Maximum Inner Product Search (MIPS), to rank the saved embeddings based on their semantic similarity with the user query, where the top \textit{k} ranked candidate data will be retrieved and concatenated with the user query. To calculate semantic similarity between any two data points, these data need to be embedded into vectors. The common embedding method can produce vectors with a length of up to 1024 using 32-bit floating-point precision (FP32). 

\textcolor{blue}{[here we need to define what is information retrieval, what is RAG, what is MIPS, what is file, document, sentence, data, etc]}


% \subsection{[Deprecated] Reshape sentence embedding under noise}
% \textcolor{red}{[do not talk too much about quantization and compression, these are not the pivotal point in this paper]}
% % \subsubsection{\textbf{Reshape sentence embedding under noise}}

% In RAG for Edge LLMs, sentence embeddings serve as indices to retrieve relevant user history data. However, when these embeddings are written into the CiM, unexpected errors may corrupt them, altering their semantic representations and shifting their positions within the high-dimensional representation space. Such corruption can result in retrieving the data which are less relevant to the user input query. Additionally, due to design and manufacturing of different CiM devices, the embeddings are normally required to be reshaped into certain size and precision to fit the device. In Figure ~\ref{fig:prelim}, we present our preliminary experiments on five datasets, which will be elaborated in \textit{section 4.1.4}, to show the impact of the noise, compression, and quantization on information retrieval performance of RAG.

% We choose \textit{all-MiniLM-L6-v2} \cite{huggingface2023}, the top widely used sentence embedding model with over 29 millions of download, as our embedding model. This model generates sentence embeddings which will be used in RAG to retrieve the appropriate information. We use accuracy as our metric, which also will be elaborated in \textit{section 4.1.3}, to measure the information retrieval performance. As shown in Figure ~\ref{fig:prelim} (a), while the compression and quantization have not been applied, the information retrieval performance on five datasets decrease along with the increase of noise \(\sigma\) on the sentence embeddings. More specifically, the performance decreases in the noise range from \(\sigma = 0.00\) to \(\sigma = 0.2\). We observe that after \(\sigma > 0.2\), the noised embeddings lead to retrieve overwhelmingly unwanted information. When \(\sigma > 0.35\), it almost prevent RAG from retrieving any appropriate information.

% From Figure~\ref{fig:prelim}(a), we note that \(\sigma = 0.1\) moderately impacts five datasets. We have chosen a noise level of \textit{0.1} for our preliminary study. In Figure~\ref{fig:prelim}(b), across compression dimensions ranging from 256 to 16, we compare the information retrieval performance using noise-corrupted embeddings (represented by solid lines) against noise-exclusive embeddings (represented by dashed lines). Applying a noise level of \(\sigma = 0.1\) to the embeddings results in an information retrieval performance decline of over 80\%. Similarly, in Figures~\ref{fig:prelim}(c) and (d), we examine the information retrieval performance under four quantization methods, comparing noise-corrupted embeddings (solid lines) to noise-exclusive embeddings (dashed lines). The results suggest that the \textit{int8} and \textit{uint8} quantization methods significantly hinder information retrieval even in the absence of noise, and the introduction of noise further degrades performance.

% From the preliminary study, we observe that the noise, compression, and quantization can compromise the information retrieval. For the noise, it corrupts the embeddings by disturbing their semantical representations. For the compression and quantization, they shrink the original representational space from \(FP32 \times 384\) by the model \textit{all-MiniLM-L6-v2} default to lower precisions and smaller dimensions. For example, the original representational space with size of \(2^{(32 \times 384)}\) can be round \(10^{3600}\) times larger than the reshaped representational space of \(int8 * 16\). When we squeeze the embeddings from the original representational space into the reshaped representational space, we inevitably alter their distance to each other which can lead to unwanted information retrieved. 

% During the information retrieval, we take the user input, which is equivalent to the anchor example in \(section 3.3\), and calculate its distances to other data in the representational space. The most semantically similar data will has the smallest distance to each other. Hence, we want the most relevant data closer to the user input than the less relevant data. Contrastive learning as we explained, can achieve this goal. 

==> 3_proposed_v0.tex <==


\section{Proposed work}


In this section, we first provide an overview of our framework. Then, we delve into the details, starting from the mechanisms that we've identified as most beneficial for the data embeddings utilized by CiM-backed RAG. We show how these mechanisms collaborate with each other to train a noise-resilient sentence embedding model. After that, we demonstrate the selective write-verify method that we use to \textcolor{red}{enhance the robustness of writing such noise-resilient embeddings into CiM} and explain the reason to use that.

\subsection{Framework Overview}

\begin{figure}[h]
  \centering
  \includegraphics[trim=0 316 585 0, clip, width=0.9\linewidth]{figures/optimize.pdf}
  \caption{Overview of the framework. Train the noise-resilient sentence transformer under our contrastive learning method. \textcolor{red}{[need a new caption]}}
  \label{fig:2}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[trim=0 454 748 0, clip, width=0.9\linewidth]{figures/overview.pdf}
  \caption{Overview of the framework. Train the noise-resilient sentence transformer under our contrastive learning method. \textcolor{red}{[need a new caption]}}
  \label{fig:2}
\end{figure}

\textcolor{red}{[change f to \(\mathcal{M}\)]}

As shown in Figure ~\ref{fig:framework}, our proposed framework utilizes contrastive learning to train the sentence transformer \(f(\cdot)\). Our framework can take labeled data and unlabeled data as the input original data, which consists of textual data related to the user. The original data will be constructed into three groups and forwarded into the input layer of \(f(\cdot)\). The embeddings from \(f(\cdot)\) will go through the post-process, a part of our data augmentation method. The post-processed embeddings will be shaped based on the constraints of \textcolor{red}{CiM device (FeFet)} to formalize the shaped embeddings. \textcolor{red}{The noise related to CiM device will be injected into these embeddings} to obtain the final embeddings. Such embeddings will can be mapped in the representation space and used to optimize \(f(\cdot)\) via contrastive learning loss.

% We use the triplet loss function in contrastive learning to train the parameters of the sentence embedding model. During training, we also incorporate compression and quantization conditions to enable the model to learn how to generate embeddings that are more suitable for such conditions.

\textcolor{purple}{move 2.3 to here}

\textcolor{purple}{noise in RAG context}

\subsection{Flexible Noise-aware Contrastive Learning}

\textcolor{red}{drop t and '}

\textcolor{blue}{In our work, we propose a flexible noise-aware contrastive learning method to improve the sentence embedding noise-resilient capability in various shapes made by compression and quantization. We construct training data into three groups including anchor, positive, and negative. While our method pull anchor and positive close and push anchor and negative further during the training, it can inject noise into the generating embeddings to calibrate the model to adapt the noise and eventually learn to generate noise-resilient embedding.}

Our contrastive learning loss function is based on Weinberger et al. \cite{weinberger2005distance}. For a set of N anchor examples \(\{x_i\}_{i=1, ..., N}\), the corresponding mini-batch consists of SN example combos after data augmentation where s is augmentation factor, which will be specified in \(section 3.3\) , \(\{\{(x_i, x_i^-, x_i^+)_s\}_{i=1, ..., N}\}_{s=1, ..., S}\), in which $x^-$ and $x^+$ are negative and positive example corresponding to $x_i$, where $x^i$ is closer to $x^+$ compared to $x^-$. Also, \(emb(x_i)\) represents the learned embedding of \(x_i\). Then the loss function \(\mathcal{L}^t\) can be defined as:

% \begin{equation}
%     \begin{gathered}
%         \mathcal{L}^t = \sum_{i=1}^{N}\mathcal{L}^t_i, \\
%         \mathcal{L}^t_i = 
        
%         \sum_ max(0, \frac{\sum_{s=1}^{S}(\text{d}(x_i, x^-_i) - \text{d}(x_i, x^+_i) + m)}{S})
%     \end{gathered}
% \end{equation}

\begin{equation}
    \begin{gathered}
        \mathcal{L}^t = \sum_{i=1}^{N} \mathcal{L}^t_i, \\
        \mathcal{L}^t_i = \frac{1}{s} \sum_{s=1}^{s} \max \left(0, \text{d}(x_i^s, x_i^{-s}) - \text{d}(x_i^s, x_i^{+s}) + m\right), \\
        \text{d}(x_a, x_b) = \text{sim}(\text{emb}(x_a), \text{emb}(x_b))
    \end{gathered}
\end{equation}
where $x_i$ is an anchor example, with its corresponding negative example $x^-$ and positive example $x^+$, where $x^i$ is closer to $x^+$ compared to $x^-$. The distance \(d(x_a, x_b)\) originally calculates the Euclidean distance between embeddings of two data \(emb(x_a)\) and \(emb(x_b)\). We use semantic similarity in our case as the distance calculation method. They formalize a set of triple examples \(\mathcal{D}_{t} = \{(x_i, x^-_i, x^+_i)\}_{i=1}^s \). 
 

% \textcolor{red}{[talk with professor]}While cross-entropy loss \textcolor{red}{[cite]} and InfoNCE \textcolor{red}{[cite]} are used in many contrastive learning works, we consider the triplet loss \cite{weinberger2005distance} because it can better reflect the distance change by setting a margin \(m\). \textcolor{red}{By alternating the margin, we can keep the trained embedding model align with noise.} The triplet loss \(\mathcal{L}'\) is defined as:

% \begin{equation}
% \begin{gathered}
%     \mathcal{L}'(x_i, x_i^-, x_i^+) = \sum_{i=1}^N \max \left(0, \text{d}(x_i, x^-_i) - \text{d}(x_i, x^+_i) + m\right), \\
%     \text{d}(x_a, x_b) = \text{sim}(\text{emb}(x_a), \text{emb}(x_b))
% \end{gathered}
% \end{equation}

% where $x_i$ is an anchor example, with its corresponding negative example $x^-$ and positive example $x^+$, where $x^i$ is closer to $x^+$ compared to $x^-$. The distance \(d(x_a, x_b)\) originally calculates the Euclidean distance between embeddings of two data \(emb(x_a)\) and \(emb(x_b)\). We use semantic similarity in our case as the distance calculation method. They formalize a set of triple examples \(\mathcal{D}_{t} = \{(x_i, x^-_i, x^+_i)\}_{i=1}^s \). 





\textcolor{red}{[TO DO: 4/24]}
\begin{itemize}
    \item use variables and formula to describe our method
    \item add our experimental results to support our choise
\end{itemize}

% \textcolor{red}{benefit 1: margin can directly related to noise sigma, while cross entropy cannot control that}

% For the triple examples \(\mathcal{D}_t\), the normal triplet loss uses margin \(m\) to pull anchor and positive examples close and push anchor and negative examples far.

% \textcolor{blue}{copy and paste the triplet loss from background to here, the original triplet loss use max and different 0}

% \textcolor{blue}{why choose triplet loss}


\subsection{Data augmentation methods}

\textcolor{green}{[change a name !!!]}

\textcolor{green}{[two ways of using profile data]}

In contrastive learning for sentence embeddings, the sentence embedding model can better learn the representations from well-constructed paired examples. Such paired examples usually consists of the original example and the augmented example made by data augmentation techniques \cite{zhang2022contrastive, wu2020clear} such as word deletion, reordering, substitution, and applying different dropout rate during embedding \cite{gao2021simcse}. Such approaches are designed to enhance the model’s ability to learn representations and produce sentence embeddings that better represent the given textual content. 

The user-generated data will be accumulated along with the usage of the Edge LLM. Such data can be used to train the embedding model. Within such data, some data have explicit labels indicate the user preference regarding certain context. One the other hand, some data have implicit labels where such data in general contain the user-related information which can also help the Edge LLM to generate user-preferred content. In our work, we propose two data augmentation methods for the two different types of data.
% In contrastive learning, it is pivotal to construct paired examples, in our case, triple examples. In the past contrastive learning for sentence embeddings, the key is to learn the appropriate representation for each sentence. 

\begin{figure}[h]
  \centering
  \includegraphics[trim=0 307 660 0, clip, width=1.\linewidth]{figures/fig_4.pdf}
  \caption{Example data augmentation method for data with explicit label and data with implicit label}
  \label{fig:ex_im_label}
\end{figure}

\subsubsection{\textbf{Data augmentation for data with explicit labels}}
For the data with explicit labels, each of the data consists of a textual content \textit{c} and its corresponding label \textit{l} which indicates the user preferred response regarding to the content \textit{c}. \textcolor{red}{As shown in Table ~\ref{tab:example}, the content-label pair can be 'abstract' to 'title', 'description' to 'tag', and 'text' to 'score'.} \textcolor{red}{(need to drop)} Such data are profile data, which we will elaborate in \textit{section 4.1.1}. Using the profile data, we will construct triple examples in the format of \((x_i, x^-_i, x^+_i)\). Given a dataset \(\mathcal{D}\) with size of $s$ profile documents, each piece of data consists of a content \(c_i\) and the corresponding label \(l_i\) where \(i \in \{1, 2, ..., s\}\). We define \(s\) as the augmentation factor. The anchor example \(x_i\) can be constructed as:
\begin{equation}
    x_i = c_i \oplus l_i, \quad \text{for } i = 1, 2, \ldots, s
\end{equation}
where \(\oplus\) denotes a concatenation operation, specifically used here to combine label and content. For each anchor data \(x_i\) with content \(c_i\), negative examples \(x^-_{i}\) can be constructed by concatenating \(c_i\) with a label \(l_k\) whose corresponding content \(c_k \neq c_i\), and \(k\) is augmentation factor that indicates the random sampling among dataset \(\mathcal{D}\) and \(i \neq k\). The negative example \(x^-_{i(k)}\) can be constructed as:
\begin{equation}
x^-_{i(k)} = c_i \oplus l_k, \quad \text{for } k = 1, 2, \ldots, k
\end{equation}
This ensures diversity in the negative examples by using different labels while maintaining the same content from the anchor.

Different from constructing anchor and its negative examples, it is challenging to construct positive examples corresponding to the anchor examples since it is more difficult to formalize semantically similar data than to formalize semantically dissimilar data. To construct positive examples, we follow the SimCSE method \cite{gao2021simcse} to add a dropout rate \(r\) into the sentence embedding model \(\mathcal{M}\). The process for constructing positive examples involves two main steps:

First, the textual positive example is formalized as:
\begin{equation}
    x^+_i = x_i, \quad \text{for } i = 1, 2, ..., s
    \label{eq:pos_label}
\end{equation}
where we align each anchor with the corresponding positive example. This step effectively duplicates the anchor data as a starting point for generating the embeddings.

Second, the embedding generation process varies based on the dropout rate applied within the model \(\mathcal{M}\). When model \(\mathcal{M}\) is utilized to generate embeddings for anchor and negative examples, the dropout rate is set to \(0\). In contrast, for generating embeddings for positive examples, a non-zero dropout rate \(r\) is used:
\begin{equation}
\begin{aligned}
    \text{emb}(x_i) &= \mathcal{M}(x_i, \text{dropout} = 0), \\    
    \text{emb}(x_i^-) &= \mathcal{M}(x_i^-, \text{dropout} = 0), \\
    \text{emb}(x^+_i) &= \mathcal{M}(x^+_i, \text{dropout} = r),
\end{aligned}
\end{equation}
where \(r \neq 0\) to induce variation in the embeddings, enhancing the model's ability to recognize semantically similar yet variably expressed content.

Given the augmentation factor \(k\), we can construct the triple data examples as:

\begin{equation}
    \mathcal{D}_{t}^{'} = \bigcup_{i=1}^s \left\{ (x_{i(k)}, x^-_{i(k)}, x^+_{i(k)}) : k = 1, 2, \ldots, k \right\}
\end{equation}

For the triplet data examples \(\mathcal{D}_{t}^{'}\), their embeddings for each augmentation \(k\) are given by:

\begin{equation}
    \mathcal{E}_{t}^{'} = \bigcup_{i=1}^s \left\{ (emb(x_{i(k)}), emb(x^-_{i(k)}), emb(x^+_{i(k))}) : k = 1, 2, \ldots, k \right\}
\end{equation}

As shown in Figure ~\ref{fig:ex_im_label}, for data with explicit labels, a content \(c\) can concatenate with its corresponding label \(l\) to formalize the positive and anchor example. That content \(c\) can also concatenate with other labels \(l'\) to formalize the negative example. The positive example can be finally obtained from the sentence embedding model with dropout rate \(r\). The anchor and negative example can be finally obtained from the sentnece embedding model with \(r = 0\). 

\input{tables/table_main}


\subsubsection{\textbf{Data augmentation for data with implicit labels}}
For data with implicit labels, each of the data consists of solely textual content \textit{c} contains the user related information. Similar to the data with explicit labels, we also use the profile data to construct triple examples in the format of \((x_i, x_i^-, x_i^+)\). Given a dataset \(\mathcal{D}\) with size of \textit{s} profile data, each piece of data consits of a content \(c_i\). The anchor data \(x_i\) can be constructed as:
\begin{equation}
    x_i = c_i, \quad \text{for } i = 1, 2, \ldots, s
\end{equation}

For each anchor data \(x_i\), constructing its corresponding negative example is not as simple as merely concatenating the content \(c_i\) with a non-corresponding label \(l_k\). In our work, since our objective is to enhance the robustness of RAG by identifying semantically similar examples, we construct the training data to emphasize the distinction between positive and negative examples. To construct negative examples, we employ a reciprocal approach with the positive examples, applying a similar method to both.

We initialize the negative example and positive example following the equation ~\ref{eq:pos_label}:
\begin{equation}
    x_i^- = x_i^+ = x_i, \quad \text{for } i = 1, 2, \ldots, s
    \label{eq:pos_anc_neg}
\end{equation}

For the positive example \(x_i^+\), it can be finalized by incorporating a dropout rate \(r\) into the sentence embedding model \(\mathcal{M}\), where a rate of \(0 < r \leq 0.2\) can generate a sentence embedding with a semantic representation similar to \(x_i\) and ensure good model training performance \cite{gao2021simcse}. Increasing the dropout rate to a higher value, such as 0.5, can distort the semantic representation of \(x_i^+\), making it dissimilar to that of \(x_i\). Training the model with such positive examples can result in poorer performance. For positive examples in training the sentence embedding model, the higher dropout rate performs more like a noise rather than a data augmentation method.

In our work, we train the sentence embedding model to generate the embeddings that can still sustain their representations under the environment with noise during \textcolor{red}{writing into CiM}. The noise can lead the original sentence embedding to represent either different semantic representations or incomplete semantic representations. As shown in Figure ~\ref{fig:ex_im_label} in the part of "Data with implicit label", the anchor example with dropout rate \(r = 0.9\) can result in a negative example that bears a corrupted representation with certain errors.


\textcolor{blue}{[need to check the grammar and content]}
\textcolor{red}{For such a negative example with corrupted representation, it is semantically dissimilar with the anchor example and positive example, although it may not express certain informative information. This situation is similar to the embedding corrupted during writing into CiM, where the corrupted embedding may not express its original representation precisely. It appears that the high dropout rate can be used to construct the negative examples, which can satisfy two points. First, the constructed negative example will be semantically different from the positive and anchor examples. Second, the constructed negative example can be treated as the CiM noise-corrupted data, which aligns with the following noise-aware training. 
}

Given the triple examples \((x_i, x_i^-, x_i^+)\), for \(i = 1, 2, ..., s\) as shown in equation ~\ref{eq:pos_anc_neg}, we have the dropout rate \(r\) for formalizing the positive examples where \(0 < r \leq 0.2\). Correspondingly, the dropout rate for formailzing the negative examples can be \(1 - r\). Given the sentence embedding model \(\mathcal{M}\), the anchor example, positive example, and negative example can be constructed as: \(\text{emb}(x_i) = \mathcal{M}(x_i, \text{dropout} = 0)\), \(\text{emb}(x_i^-) = \mathcal{M}(x_i^-, \text{dropout} = 1 - r)\), and \(\text{emb}(x^+_i) = \mathcal{M}(x^+_i, \text{dropout} = r)\).

% \begin{equation}
%     \begin{aligned}
%     \text{emb}(x_i) &= \mathcal{M}(x_i, \text{dropout} = 0), \\    
%     \text{emb}(x_i^-) &= \mathcal{M}(x_i^-, \text{dropout} = 1 - r), \\
%     \text{emb}(x^+_i) &= \mathcal{M}(x^+_i, \text{dropout} = r),
% \end{aligned}
% \end{equation}



% \subsection{Noise-aware CiM-efficient training}
% \subsubsection{\textbf{Embedding compression and quantization}}
% \subsubsection{\textbf{Noise-aware sentence embedding}}

% \textcolor{red}{why change noise, this framework can fit into any device}




% \subsection{Algorithm}

% auto search for the appropriate margin, dropout, based on noise, we might need an alogrithm

% this is for getting the correct margin based on noise


==> 4_experiments_v0.tex <==
\section{Experimental Evaluation}

\subsection{Experimental Setup}\label{sect:setup}
% We first explain the datasets used in the experiments, the settings under different experiments, evaluation methods, the baselines, and how the different experiments support our work.

\input{tables/table_1}
% \textcolor{red}{need source to make the noise practical}

\subsubsection{\textbf{Datasets.}} \textcolor{red}{[should we use their name in LaMP, or their original names?]} To demonstrate our robust CiM-backed RAG, we employ five datasets with different tasks and domains, including Citation Identification \cite{salemi2023lamp}, Movie Tagging \cite{harper2015movielens}, Product Rating \cite{ni2019justifying}, News Headline Generation \cite{misra2022news}, and DBLP-Citation-network V14 \cite{tang2008arnetminer} to evaluate the proposed framework. The data in each dataset consists of query data and profile data. In our evaluation, the profile data will be used to formalize user history, and the profile corresponding query data will be used as the user input. The first three datasets contain binary, five-class, and fifteen-class classification tasks respectively. The last two datasets contain text generation tasks. In the Citation Identification dataset, every piece of query data consists of a paper title and two references, and the correct reference is provided. RAG can use the profile data, corresponding to the paper titles with their detailed contents, to choose the appropriate reference. In the Movie Tagging data set, each query data contains a description of a movie, and RAG can use a similar description and its corresponding tag in the profile data to tag the query data. The Product Rating dataset has a similar structure as the Movie Tagging dataset. In News Headline Generation and DBLP datasets, each query data contains an abstract, which can be summarized into a title. The RAG can use a similar abstract and its corresponding title in profile data to generate the title for query data. All five datasets have labels in query data.

\input{tables/table_cim_info}


\begin{figure*}[ht]
  \centering
  % First row of figures
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=1\textwidth]{figures/fig_7_a.pdf}
    \caption{Citation on Gemma-2b}
    \label{fig:a}
  \end{subfigure}
  % \hfill % space between the subfigures
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=1\textwidth]{figures/fig_7_b.pdf}
    \caption{Citation on Phi-2}
    \label{fig:b}
  \end{subfigure}
  % \hfill % space between the subfigures
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=1\textwidth]{figures/fig_7_c.pdf}
    \caption{Citation on Mistral-7B}
    \label{fig:c}
  \end{subfigure}
  % Second row of figures
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=1\textwidth]{figures/fig_7_d.pdf}
    \caption{Citation on Llama-2-3B}
    \label{fig:d}
  \end{subfigure}
  % \hfill % space between the subfigures
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=1\textwidth]{figures/fig_7_e.pdf}
    \caption{Movie on Gemma-2b}
    \label{fig:e}
  \end{subfigure}
  % \hfill % space between the subfigures
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=1\textwidth]{figures/fig_7_f.pdf}
    \caption{Movie on Phi-2}
    \label{fig:f}
  \end{subfigure}
    % \hfill % space between the subfigures
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=1\textwidth]{figures/fig_7_g.pdf}
    \caption{Movie on Mistral-7B}
    \label{fig:g}
  \end{subfigure}
  % \hfill % space between the subfigures
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=1\textwidth]{figures/fig_7_h.pdf}
    \caption{Movie on Llama-2-3B}
    \label{fig:h}
  \end{subfigure}
  \caption{Compare the performance our framework with four baselines \textcolor{red}{with different LLMs} with default \(\sigma = 0.1\), given dataset \(Citation\) and \(Movie\). }
  \label{fig:four_LLMs}
\end{figure*}

\subsubsection{\textbf{Default Experimental Setting.}} 

\textcolor{red}{ baseline4 is vanilla}

Our framework choose \textit{all-MiniLM-L6-v2} \cite{huggingface2023} as the sentence embedding model. As shown in Figure ~\ref{fig:2}, the sentence embedding model convert the user query and past user data from user database from textual format to numerical representations. For each dataset, we randomly select 2000 data as the anchor examples. To examine the data augmentation method for data with explicit labels, we set the augmentation factor \(k = 5\) to obtain 10000 negative examples where one anchor example can generate five negative examples. We set dropout rate as 0.1 to obtain the positive examples while maintain it as 0 when process anchor and negative examples. To examine the data augmentation method for data with implicit labels, we set dropout rate for positive examples as 0.1 and dropout rate for negative examples as 0.9. To align with the experiments for explicit labeled data, we also create five positive and five negative examples for each anchor example. For the experimental results, we run five times and get the average. The LLM, in Figure ~\ref{fig:2}, takes the MIPS-fetched data and the user query to generate response.

\textcolor{red}{this part is how to set up our framework. depends on the variable names, I set the sigma as 0.1, shape all embeddings into 64 * int8, the learning rate is 2e-5. (I will expand this part later)}

% In our framework, we choose a widely-used pretrained sentence embedding model \textit{all-MiniLM-L6-v2} \cite{huggingface2023} as the core model, which further will be altered and fine-tuned to generate the CiM-friendly data embedding. As shown in Figure ~\ref{fig:2}, other than the sentence embedding model, LLM takes the searched user data and the user query as the input to generate the output. In our experiments, we choose Gemma-2B developed by Google \cite{team2024gemma}, the up-to-date newest LLM with model weights size of 4.95G which can fit to edge device, as the LLM to generate response to the user. For each dataset, we randomly sample 500 query data where each query data corresponds to 100 profile data as our training data. To evaluate our framework, in each dataset we choose 200 query data where each query data corresponds to the same amount of profile data as our test data.




In all experiments, we adhere to the device variation model previously described. The specific parameters are abstracted and then simplified from three representative NVM devices, two of them are resistive random-access memory (RRAM) devices extracted from~\cite{yao2020fully, liu2023architecture} and the other is a ferroelectric field effect transistor (FeFET) device extracted from~\cite{wei2022switching}. We name them $RRAM_1$, $RRAM_4$ and $FeFET_2$, respectively. We also extrapolate the modeling data to obtain two synthesized $FeFET_3$ and $FeFET_6$ devices. Detailed device modeling results are demonstrated in Table~\ref{tab:var}. A $x$-level device means this device can represent $x$ distinct values and $\sigma_{L_2} = 0.03$ means the variation of this device is 0.01 when it is representing the value 2.

Embedding vectors are quantized and then each element is mapped to multiple NVM devices. For example, if an embedding vector contains values quantized to unint8, when it's mapped to 4-level (2-bit) devices like $FeFET_2$, each element of this vector is represented by 4 devices.


\subsubsection{\textbf{Evaluation Methods.}}

\textcolor{red}{[also compute the MIPS accuracy]}

Our first three datasets examine the model classification capability, and the rest of two datasets examine the text generation capability. Dataset \(Citation\) and \(Movie\) has two and fifteen labels respectively. We can examine the binary and multiclass classification capabilities of the LLMs enhanced by our framework. In this way, we use accuracy to examine the ability of the models to correctly classify instances across different classes, and we use F1 score to examine the balance between precision and recall in classification tasks. For dataset \(Rating\), while it has five labels and also examine the multiclass classification, we use mean absolute error (MAE) and root mean square error (RMSE) to evaluate from from a regression perspective \cite{chai2014root}. For MAE, it measures the average magnitude of errors in the predictions, providing a straightforward assessment of the model's overall accuracy in predicting the rating values. For RMSE, it captures the square root of the average squared differences between predicted and actual ratings, offering a metric sensitive to larger errors, which can highlight significant discrepancies between the model's predictions and true values. For dataset \(News\) and \(DBLP\), as shown in Table ~\ref{tab:example}, their labels are sentences. Such datasets examine the text generation capabilities. We use ROUGE-1 and ROUGE-L to evaluate the overlap between generated texts and reference texts \cite{lin2004rouge}, capturing both the precision and recall of individual words (ROUGE-1) and the longest matching sequence (ROUGE-L), ensuring a comprehensive evaluation of the text generation quality. For accuracy, F1, ROUGE-1 and ROUGE-L, their higher values reflect the better performance. For MAE and RMSE, their lower value represent the better performance.


\subsubsection{\textbf{Baselines.}}

As this is the first work to improve the RAG robustness on Edge-based CiM, we do not have state-of-the-art for comparison. As such we construct a few vanilla baselines from the past noise mitigation methods originally designed to boost DNN robustness. \(Baseline1\) comes from selective write verify \cite{yan2022swim}. While it originally utilize the second derivation to evaluate the device variation impact on neural network weights, we use the second derivation to measure the embedding deviation between the ground truth embedding and the embedding under device variation. \(Baseline2\) comes from CxDNN \cite{jain2019cxdnn}. While they use compensation factor to improve the robustness of vector-matrix multiplication, we use the compensation factor the calibrate the embedding impacted by device variation. \(Baseline3\) comes from CorrectNet \cite{eldebiky2023correctnet}. While they utilize the cross entropy loss and regularization to improve the robustness of neural networks in CiM, we use the cross entropy loss the regularization as the loss function to calibrate the device output embedding. Additionally, we utilize raw RAG as our \(Baseline4\). The raw RAG contains no noise mitigation methods. 





\subsection{Results}

\textcolor{red}{We start with cmpare the MIPS accuracy [done]}

\textcolor{red}{Then we present a comprehensive study of RAG, which contains MIPS and LLM, chose Gemma-2 [done]}

\textcolor{red}{Additionally, choose two datasets, we examine four different LLMs. Why? We want to show that MIPS results can impact all different LLMs [done]}

\textcolor{red}{Finally, we examine the impact of device variation}


We start with comparing the performance of RAG on five CiM devices (sigma is 0.1) and the raw RAG, where no embedding model fine-tuning or device variation injection is applied. The RAG utilized Gemma-2B as its LLM module. The results are presented in Table ~\ref{tab:prelim_1}. From the table we can see the CiM device variation can reduce the RAG performance more than 50\%, compared with the raw RAG. 

\input{tables/table_prelim_1}

Next, we present a comprehensive experiment set, to compare our framework, one for explicit labels (\(ours-ex\)) and one for implicit labels (\(ours-im\)), with selective write verify (\(Baseline1\)), CxDNN (\(Baseline2\)), CorrectNet (\(Baseline3\)), and raw RAG (\(Baseline4\)). The results are presented in Table ~\ref{tab:main}. The comprehensive table present how our framework can mitigate the different device variation with respect to different datasets. Given the same datasets, we can observe that each device variation can largely compromise the RAG robustness. For example, the RAG performance for Citation dataset on Device-2 can range from 0.18 to 0.48, while our framework can boost the accuracy performance of Citation dataset above 0.5 for all five devices.

In addition, we evaluate the impact of different LLMs on the performance of our framework. As Figure ~\ref{fig:2} shown, the LLM takes the concatenation of MIPS searched data and user query as the input and generates the response regarding the user query. Since different LLMs may have different response given the same query, we select four emerging edge-friendly medium-size LLMs in our experiments to examine the performance of our framework. Gemma-2B \cite{team2024gemma} is a new SOTA open model introduced by Google, with 4.95G model weights. According to Google, Gemma can outperform the same sized Llama-2 in reasoning capabilities. Hence, we also use Llama-2-3B \cite{openlm2023openllama}, one of the earliest open LLMs introducted by Meta, with 6.85G model weights. Similarly, Phi-2 \cite{gunasekar2023textbooks} released by Microsoft, is a powerful small LLM with 5G model weights. Additionally, Mistral-7B-GPTQ \cite{jiang2023mistral} made by Mistral AI, is a well-performed LLM after Llama model. We select dataset \(Citation\) and dataset \(Moive\). We use the default experimental setting with sigma = 0.1 and use CiM Device-1 as the experimental environment. The results are shown on Figure ~\ref{fig:four_LLMs}. It appears that our framework can outperform each baseline across five CiM devices. Besides, the performance of each baseline on the same dataset can be largely different given different device, while our framework can produce a more robust performance. 

When use a method to improve the RAG robustness, the RAG performance is expected to be constant on different CiM devices. We further analyze the robustness of our framework and the baselines using standard deviation. 

\input{tables/table_std_temp}

\textcolor{red}{[continue work...]}


To demonstrate our work has effectiveness and efficiency, we have Figure ~\ref{fig:overhead} to show the overhead and latency of each method. We have Table ~\ref{tab:main} to show our work can outperform the past SOTA in five datasets with commonly-accepted metrics. On two datasets, we also exam the four baselines and our work on five CiM devices, with four popular medium sized LLMs, as shown in Figure ~\ref{fig:four_LLMs}

Furthermore, we present ablation study. From Figure ~\ref{fig:four_LLMs}, we observe Mistral-7B has in average decent performance across four baselines across five devices. Hence, we choose Mistral-7B and study how our framework can handle different sigmas (0.025, 0.05, 0.075, 0.1, 0.125, 0.15). We choose Device-1 as the experimental platform. For the dataset, we choose \(DBLP\). This is ablation study 1, see Figure ~\ref{fig:ablation1} (\textcolor{red}{[the figure is a sample figure, we are still running experiments to get the results...]})

\begin{figure}[h]
  \centering
  \includegraphics[width=0.7\columnwidth]{figures/fig_8.pdf}
  \caption{Different device variation for our work \textcolor{red}{use RAG}}
  \label{fig:ablation1}
\end{figure}
\textcolor{red}{make line more readable, use rouge}

In Figure ~\ref{fig:overhead}, we study the overhead. \textcolor{red}{[the figure is a sample, we will get results soon...]}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.7\columnwidth]{figures/fig_6.png}
  \caption{overhead for each method}
  \label{fig:overhead}
\end{figure}

\textcolor{red}{here I am going to add more details including explanation and analysis. But I will add some other experimental chart first}





==> tables/table_1.tex <==
\begin{table}[h]
\centering
\footnotesize
\caption{Sample of profile data for each dataset \textcolor{red}{[drop]}}
\begin{tabularx}{\linewidth}{cl>{\raggedright\arraybackslash}X}
\toprule
\multicolumn{2}{l}{\textbf{Dataset}} & \textbf{Profile Data} \\
\midrule
\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{Citation}}} 
    & [label] title & "Infrastructure tradeoffs for sensor networks" \\
    & abstract      & "In a sensor network, the infrastructure plays a vital role in determining the performance of the network. We study the effect of infrastructure decisions on a sensor network."\\

\midrule
\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{Moive}}} 
    & [label] tag   & "classic" \\
    & description   & "Humanity finds a mysterious object buried beneath the lunar surface and sets off to find its origins with the help of HAL 9000, the world's most advanced super computer." \\

\midrule
\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{Rating}}} 
    & [label] score & "3" \\
    & text          & "The recipes sound great and many of them require basic ingredients that are on hand in most kitchens. I've enjoyed slow cooker recipes and I'll definitely try some of these." \\

\midrule
\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{News}}} 
    & [label] title & "Five Things Women Can Do Today to Move Past Divorce" \\
    & text          & "I know it sounds trite, but now you have the freedom to be you and to let it reflect in your home, surroundings and daily activities. Embrace it, run with it and most of all enjoy it." \\

\midrule
\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{DBLP}}} 
    & [label] title & "A parallel algorithm for logic simulation on networks" \\
    & abstract      & "The authors present a parallel algorithm for logic simulation of VLSI circuits. It is implemented on a network of transputers connected in a ring topology." \\
    
\bottomrule
\end{tabularx}
\label{tab:example}
\end{table}


==> tables/table_std_temp.tex <==

\begin{table}[htbp]
\caption{RAG performance using Gemma-2B on different CiM devices. Examine \(Baseline4\).}
    \centering
    \footnotesize
    \begin{tabularx}{\columnwidth}{c*{5}{Y}} 
        \toprule
        \textbf{Dataset} & \textbf{Citation} & \textbf{Movie} & \textbf{Rating} & \textbf{News} & \textbf{DBLP} \\
        \midrule
        Baseline1  & 0.36 $\pm$ 0.12 & 0.15 $\pm$ 0.03 & 0.38 $\pm$ 0.03 & 0.05 $\pm$ 0.02 & 0.15 $\pm$ 0.04 \\
        Baseline2  & 0.44 $\pm$ 0.03 & 0.16 $\pm$ 0.06 & 0.37 $\pm$ 0.06 & 0.07 $\pm$ 0.01 & 0.16 $\pm$ 0.02 \\
        Baseline3  & 0.43 $\pm$ 0.03 & 0.12 $\pm$ 0.03 & 0.41 $\pm$ 0.07 & 0.06 $\pm$ 0.01 & 0.18 $\pm$ 0.02 \\
        Baseline4  & 0.41 $\pm$ 0.10 & 0.13 $\pm$ 0.03 & 0.39 $\pm$ 0.03 & 0.06 $\pm$ 0.02 & 0.18 $\pm$ 0.02 \\
        Ours-ex    & 0.55 $\pm$ 0.02 & 0.23 $\pm$ 0.04 & 0.30 $\pm$ 0.02 & 0.10 $\pm$ 0.01 & 0.20 $\pm$ 0.01 \\
        Ours-im    & 0.54 $\pm$ 0.01 & 0.23 $\pm$ 0.04 & 0.26 $\pm$ 0.03 & 0.10 $\pm$ 0.01 & 0.22 $\pm$ 0.01 \\

        \bottomrule
    \end{tabularx}
    \label{tab:std}
\end{table}


